To Forget or Not? Towards Practical Knowledge Unlearning for Large Language Models

Large Language Models (LLMs) trained on extensive corpora inevitably retain sensitive data, such as personal privacy information and copyrighted material. Recent advancements in knowledge unlearning involve updating LLM parameters to erase specific knowledge. However, current unlearning paradigms are mired in vague forgetting boundaries, often erasing knowledge indiscriminately. In this work, we introduce KnowUnDo, a benchmark containing copyrighted content and user privacy domains to evaluate if the unlearning process inadvertently erases essential knowledge. Our findings indicate that existing unlearning methods often suffer from excessive unlearning. To address this, we propose a simple yet effective method, MemFlex, which utilizes gradient information to precisely target and unlearn sensitive parameters. Experimental results show that MemFlex is superior to existing methods in both precise knowledge unlearning and general knowledge retaining of LLMs. Code and dataset are released at https://github.com/zjunlp/KnowUnDo.

==> tab/backup.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{2\columnwidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
Models & \multicolumn{3}{c}{Forget Set} & \multicolumn{2}{c}{Retain Set} & \multicolumn{5}{c}{Downstream Task Accuracy} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-11}
 & ACC\textsuperscript{\textdagger} & PPL\textsuperscript{\textdagger} & MIA & ACC\textsuperscript{\textdagger} & PPL\textsuperscript{\textdagger} & MMLU & ARC & TruthfulQA & WMDP & Avg. \\
\midrule
Vanilla Model & 69.02 & 3.65 & 50.77 & 52.68 & 9.24 & 63.37 & 68.49 & 16.46 & 33.59 & 45.48 \\
Approximate Retrain & 68.98 & 3.69 & - & - & - & - & - & - & - & - \\
Gradient Ascent & 68.79 & 3.70 & 52.66 & 52.66 & 9.26 & 63.45 & 68.77 & 15.85 & 34.04 & 45.53 \\
Fine-tuning with Random Labels & 68.92 & 3.69 & 52.67 & 52.67 & 9.25 & 63.37 & 68.38 & 14.02 & 32.22 & 44.50 \\
Unlearning with Adversarial Samples & 68.87 & 3.69 & 50.52 & 52.68 & 9.25 & 63.32 & 68.74 & 15.24 & 33.13 & 45.11 \\
\midrule
Gradient Ascent + Descent on retain set &  &  &  &  &  &  &  &  &  &  \\
- Descent on in-distribution data & 68.87 & 3.69 & 50.18 & 52.66 & 9.26 & 63.32 & 68.52 & 15.24 & 33.74 & 45.21 \\
- Descent on general data & 68.81 & 3.69 & 50.33 & 52.93 & 9.04 & 63.40 & 67.87 & 15.24 & 33.13 & 44.91 \\
Gradient Ascent + KL divergence &  &  &  &  &  &  &  &  &  &  \\
- KL on in-distribution data & 68.82 & 3.69 & 50.29 & 52.65 & 9.27 & 63.40 & 68.57 & 15.24 & 33.89 & 45.28 \\
- KL on general data & 68.79 & 3.70 & 50.25 & 52.65 & 9.27 & 63.27 & 68.38 & 15.85 & 33.81 & 45.33 \\
\bottomrule
\end{tabular}
}
\caption{Overall results of unlearning LLaMA-2-7B-Chat on a subset of pre-training data (500 arXiv papers)}
\end{table*}
